Simultaneous determination of the cosmic birefringence and miscalibrated polarization angles II: Including cross frequency spectra

We develop a strategy to determine the cosmic birefringence and miscalibrated polarization angles simultaneously using the observed $EB$ polarization power spectra of the cosmic microwave background and the Galactic foreground emission. We extend the methodology of Y. Minami et al. (Prog. Theor. Exp. Phys. $\mathbf{2019}$, 083E02, 2019), which was developed for auto frequency power spectra, by including cross frequency spectra. By fitting one global birefringence angle and independent miscalibration angles at different frequency bands, we determine both angles with significantly smaller uncertainties (by more than a factor of two) compared to the auto spectra.

==> PlanckHFI.tex <==
We apply our methodology to real microwave sky observed by Planck HFI.
We use Planck PR3 maps which are reprocessed in 2018.

\begin{table}
	\centering
	\caption{}
	\label{tab:PlanckSpec}
	\begin{tabular}{ccc}
		$\nu$ (GHz) & $f_\mathrm{sky}$ & 		
	\end{tabular}
\end{table}

\subsection{Sky map and mask}
In this study, 
we use cross correlation of two maps which are the Planck map divided in half (the Planck half-mission maps, HM)
to reduce the correlated systematics and bias from auto correlation noise.
We apply three types of selection to create mask for each HM map,
\begin{enumerate}
	\item  Removal of bad pixels : In HM maps, there are some sky pixels where detectors did not see. 
	We mask the pixels.
	\item  Removal of low resolution effects from CO foreground templates:  To reduce the noise of the CO bandpass templates, the bandpass correction have been applied to Planck maps. 
	However, the difference between the resolution of CO simulated map ($\mathrm{N}_\mathrm{side}=128$) and that of the HM maps ($\mathrm{N}_\mathrm{side}=2048$) gives bias.
	To reduce the bias, we mask the the very bright regions where  the bias level is larger than $1\%$ of the variance of the noise level~\cite{Planck2018HFI}.
	\item Removal of bright point source: We mask the polarized point sources to remove \textcolor{red}{spurious?} $EB$ correlations.
	We remove sources with polarization detection significance levels are equals to or greater than $99.97\%$. 
\end{enumerate}

We apodize the mask with $0.5\deg$

\subsection{From map to power spectra}

We use the public code ``NaMaster''

We remove the leakage from Intensity to polarization ($I\to P$ leakage)


